Tight lower bounds for the complexity of multicoloring

In the multicoloring problem, also known as ($a$:$b$)-coloring or $b$-fold coloring, we are given a graph G and a set of $a$ colors, and the task is to assign a subset of $b$ colors to each vertex of G so that adjacent vertices receive disjoint color subsets. This natural generalization of the classic coloring problem (the $b=1$ case) is equivalent to finding a homomorphism to the Kneser graph $KG_{a,b}$, and gives relaxations approaching the fractional chromatic number. We study the complexity of determining whether a graph has an ($a$:$b$)-coloring. Our main result is that this problem does not admit an algorithm with running time $f(b)\cdot 2^{o(\log b)\cdot n}$, for any computable $f(b)$, unless the Exponential Time Hypothesis (ETH) fails. A $(b+1)^n\cdot \text{poly}(n)$-time algorithm due to Nederlof [2008] shows that this is tight. A direct corollary of our result is that the graph homomorphism problem does not admit a $2^{O(n+h)}$ algorithm unless ETH fails, even if the target graph is required to be a Kneser graph. This refines the understanding given by the recent lower bound of Cygan et al. [SODA 2016]. The crucial ingredient in our hardness reduction is the usage of detecting matrices of Lindstr\"om [Canad. Math. Bull., 1965], which is a combinatorial tool that, to the best of our knowledge, has not yet been used for proving complexity lower bounds. As a side result, we prove that the running time of the algorithms of Abasi et al. [MFCS 2014] and of Gabizon et al. [ESA 2015] for the r-monomial detection problem are optimal under ETH.

==> detecting.tex <==

The crux of our reduction relies on the use of so called \emph{$d$-detecting families}, a combinatorial object that allows us to save a logarithmic factor in size.
They can be introduced by the following riddle: given $n$ coins with integer weights in $[d]$ (for some fixed integer $d$), how many weighings do we need to uniquely determine all their weights?
Each weighing gives us the exact total weight of any chosen subset of coins.

Clearly $n$ weighings, taking each coin individually, is enough.
If the weights were unbounded, elementary linear algebra implies that $n$ is also necessary.
Here, quite surprisingly, $\Oh(\frac{n}{\log_d n})$ weighings are enough.
This matches the information-theoretic lower bound: intuitively, each weighing gives us $\lg nd$ bits of information (one number between $0$ and $n(d-1)$), while for the final answer we need $n \lg d$ bits in total ($n$ numbers between $0$ and $d-1$), so at least $\frac{n \lg d}{\lg nd}$ weighings are needed.
The subsets of coins to weigh can be fixed before any weighing is done, giving the following definition.


\begin{definition}\label{def:uniftest}
%For any $\alpha \in \mathbb{N}$, $\mathcal{F}_\alpha$ is the family of all functions $f : \mathcal{U} \rightarrow \{0,1,\ldots,\alpha-1\}$ for some set $\mathcal{U}$.
A \emph{$d$-detecting family} for a set $\mathcal{U}$ is a family $\mathcal{F} \subseteq 2^\mathcal{U}$ of subsets of $\mathcal{U}$ such that for every two functions $f,g:\mathcal{U}\to[d]$, $f \neq g$, there is a set $S$ in the family such that $\sum_{x \in S} f(x) \neq \sum_{x \in S} g(x)$.
\end{definition}

A deterministic construction of sublinear, $d$-detecting families was given by Lindstr{\"o}m~\cite{lindstrom1965combinatorial}, together with a proof that the constant factor 2 in the family size cannot be improved.

\begin{theorem}[\cite{lindstrom1965combinatorial}]\label{th:uniftest}
For every constant $d \in \mathbb{N}$ and finite set $\mathcal{U}$, there is a $d$-detecting family $\mathcal{F}$ on $\mathcal{U}$ of size $\frac{2|\mathcal{U}|}{\log_d |\mathcal{U}|} \cdot \left(1 + o(1)\right)$. Furthermore, $\mathcal{F}$ can be constructed in time polynomial in $|\mathcal{U}|$.
\end{theorem}

See also Grebinski \& Kucherov~\cite{GrebinskiK00}, and Bshouty~\cite{Bshouty09} for other constructions, generalizations, and overviews of similar results.
Note that the expression $\sum_{x \in S} f(x)$ is just the product of $f$ as a vector in $[d]^{|\mathcal{U}|}$ with the characteristic vector of $S$ -- hence instead of subset families, Lindstr{\"o}m speaks of \emph{detecting vectors}, while later works see them as \emph{detecting matrices}, that is, $(0,1)$-matrices with these vectors as rows (which define an injective functional on $[d]^{|\mathcal{U}|}$ despite having few rows).
Similar definitions occur when studying query complexity, e.g. as in the popular Mastermind game~\cite{Chvatal83}.

While known polynomial deterministic constructions of detecting families involve some number theory or fourier analysis, their existence can be argued with an elementary probabilistic argument.
Intuitively, a random subset $S\subseteq \mathcal{U}$ will distinguish two distinct functions $f,g:\mathcal{U}\to[d]$ (meaning $\sum_{x \in S} f(x) \neq \sum_{x \in S} g(x)$) with probability at least $\frac{1}{2}$ -- this is because any $x$ where $f$ and $g$ disagree is taken or not taken into $S$ with probability $\frac{1}{2}$, while sums over $S$ cannot agree in both cases simultaneously, as they differ by $f(x)$ and $g(x)$ respectively.
There are $d^{n} \cdot d^{n}$ function pairs to be distinguished.
In any subset of pairs, at least half are distinguished by a random set in expectation, thus at least one such set exists. 
Repeatedly finding such a set for undistinguished pairs, we get $|\log_{\frac{1}{2}} (d^{n} \cdot d^n)| = \Oh(n \log d)$ sets that distinguish all functions.
More strongly though, when two functions differ on more values, the probability of distinguishing them increases significantly -- so we need fewer random sets to distinguish all pairs of distant functions. On the other hand, there are few function pairs that are close, so we need few random sets to distinguish them all as well.
This allows to show that in fact $\Oh(\frac{n}{\log_d n})$ random sets are enough to form a $d$-detecting family with positive probability~\cite{GrebinskiK00}.

%\begin{proof}
%Randomly sampling subsets (each elements with probability $\frac12$).
%
%\newcommand\nU{\ensuremath{b}}
%Let $\nU = |\mathcal{U}|$.
%Let us call a function $f : \mathcal{U} \to [\alpha]$ \emph{small} iff $\left|f^{-1}(\{i\})\right| \leq \sqrt{\nU}$ for all $i\neq \beta$.
%The number of small functions is at most $\binom{\nU}{\sqrt{\nU}}^{\alpha-1} = 2^{\Oh(\sqrt{\nU} \log \nU)}$.
%
%Let $S \subseteq \mathcal{U}$ be a random subset of $\mathcal{U}$, with each element independently with probability $\frac12$.
%If $f \not\equiv \beta$, then $f(S)\neq \beta \cdot |S|$ with probability at least $\frac12$ (because if $x$ is any element such that $f(x)\neq \beta$, then at most one set of $S\setminus\{x\}, S\cup \{x\}$ can have $f(S)=\beta \cdot |S|$...).
%
%If $f$ is large and $f\not\equiv \beta$, then $f(S) =\beta \cdot |S|$ with probability at most $\frac{1}{c \cdot \nU^{1/4}}$.
%Indeed, since $f$ is large, there is an  $i \in [\alpha]$, $i\neq \beta$, such that $|f^{-1}(\{i\})| > \sqrt{\nU}$. Let $U_i = f^{-1}(\{i\})$.
%Then for any fixed value of $S \setminus U_i$, we can have $f(S) = \beta \cdot |S|$ only if $f(S \cap U_i) = \beta \cdot |S| - f(S \setminus U_i)$, which implies $|S \cap U_i| \cdot i = \beta \cdot |S \cap U_i| + \beta \cdot |S \setminus U_i| - f(S \setminus U_i)$ and thus $|S \cap U_i| = c$, for $c =(\beta \cdot |S \cap  \setminus U_i| - f(S \setminus U_i)) / (i - \beta)$.
%This happens with probability exactly $\binom{|U_i|}{c}/2^{|U_i|} \leq \binom{|U_i|}{|U_i|/2}/2^{|U_i|} < \frac{1}{\sqrt{\pi \cdot |U_i| / 2}} < \frac{1}{\sqrt{|U_i|}} < \frac{1}{\nU^{1/4}}$ for any fixed value of $S \cap X$ and thus globally...
%%I checked the exact inequalities, cite "Computationally Efficient Bounds for the Catalan Numbers" if you must.
%% http://www.sciencedirect.com/science/article/pii/S0195669886800245
%
%\end{proof}

\bigskip
Let us now sketch how detecting families are used in our reductions.
Our aim is to reduce an instance $\phi$ of 3-SAT with $n$ variables into an instance $G$ of $a$:$b$-coloring with $\Oh(\frac{n}{\log b})$ vertices.
The $a$:$b$-colorings will correspond to truth assignments for variables of $\phi$ and a choice (a subset) of satisfied literals (made positive by the assignment).
%Clauses will be grouped into sets of size $b$ such that two clauses in a common group share no variables, essentially -- 
Let us consider a group $C$ of $b$ clauses of $\phi$.
For any set $S\subseteq C$ of clauses, by adding an appropriate vertex to $G$, we will be able to add a constraint expressing that \emph{exactly $|S|$ satisfied literals were chosen in clauses of $S$}.
Since many literals can be made positive in a single clause, other clauses from $S$ can still be unsatisfied.

To express that \emph{every} clause is satisfied, we could of course add such a constraint for each clause individually, but that would require $|C|=b$ vertices.
To introduce only $\Oh(\frac{b}{\log b})$, we shall introduce a vertex for every set $S$ of a $4$-detecting family for $C$.
If the function $f: C \to \{0,1,2,3\}$ describes how many literals are satisfied in each clause, the introduced vertices guarantee that $\sum_{x \in S} f(x) = |S| = \sum_{x \in S} 1$ for every $S$ in the detecting family.
By definition, this implies $f(c) = 1$ for all $c \in C$ --- that is, every clause of $C$ is satisfied.

%\todo[inline]{Use a corollary like the following if you want. MW}
%We therefore use 4-detecting families only in the following case, which can be shown not to be significantly weaker though (up to choices of constants).
%\begin{corollary}\label{cor:detecting}
%	For every $b\in\mathbb{N}$, there is a family $\mathcal{F}\subseteq 2^{[b]}$ of size $\Oh(\frac{b}{\log b})$ such that for any function $f:[b]\to\{0,1,2,3\}$,
%	if $\sum_{x\in S} f(x) = |S|$ for all $S\in\mathcal{F}$, then $f\equiv 1$.
%	Furthermore, $\mathcal{F}$ can be constructed in time polynomial in $b$.
%\end{corollary}


==> fig-kneser.tex <==
\tikzset{ %
	e/.style={very thick},
	C/.style={circle,draw=black,inner sep=0pt,minimum size=30pt,fill=white},
	s/.style={circle,draw=none,inner sep=0pt,minimum size=9pt},
	sn/.style={s,fill=black!10},
	s0/.style={s,fill=red!80!black},
	s1/.style={s,fill=blue},
	s2/.style={s,fill=green},
	s3/.style={s,fill=violet},
	s4/.style={s,fill=orange},
%	V/.style={circle,draw=black,inner sep=0pt,minimum size=5pt,fill=black},
%	L/.style={V, fill=gray!80!black},	
%	v/.style={circle,draw=black,inner sep=0pt,minimum size=8pt,fill=blue!30},
%	u/.style={circle,draw=black,inner sep=0pt,minimum size=8pt,fill=yellow!25!red!70},	
%	w/.style={circle,draw=black,inner sep=0pt,minimum size=8pt,fill=yellow!40},		
%	vg/.style={fill=blue!25},
%	cla/.style={fill=yellow!60!brown!90!gray!30!white},
%	clg/.style={draw=black!30,fill=yellow!60!brown!90!gray!50!white}
}
\begin{tikzpicture}
	\node[C] (v0) at (0*360/5:1.5) {};	
	\node[C] (v1) at (1*360/5:1.5) {};
	\node[C] (v2) at (2*360/5:1.5) {};	
	\node[C] (v3) at (3*360/5:1.5) {};	
	\node[C] (v4) at (4*360/5:1.5) {};
	\node[C] (w0) at (0*360/5:3.0) {};	
	\node[C] (w1) at (1*360/5:3.0) {};
	\node[C] (w2) at (2*360/5:3.0) {};	
	\node[C] (w3) at (3*360/5:3.0) {};	
	\node[C] (w4) at (4*360/5:3.0) {};	
	\draw[e] (v0) -- (v2) -- (v4) -- (v1) -- (v3) -- (v0);
	\draw[e] (w0) -- (w1) -- (w2) -- (w3) -- (w4) -- (w0);
	\draw[e] (v0) -- (w0) (v1) -- (w1) (v2) -- (w2) (v3) -- (w3) (v4) -- (w4);
	
	\begin{scope}[shift={(0*360/5:1.5)}]
		\node[sn] at (0*360/5:0.3) {};
		\node[sn] at (1*360/5:0.3) {};
		\node[s2] at (2*360/5:0.3) {};
		\node[s3] at (3*360/5:0.3) {};
		\node[sn] at (4*360/5:0.3) {};								
	\end{scope}
	
	\begin{scope}[shift={(1*360/5:1.5)}]
		\node[sn] at (0*360/5:0.3) {};
		\node[sn] at (1*360/5:0.3) {};
		\node[sn] at (2*360/5:0.3) {};
		\node[s3] at (3*360/5:0.3) {};
		\node[s4] at (4*360/5:0.3) {};								
	\end{scope}
	
	\begin{scope}[shift={(2*360/5:1.5)}]
		\node[s0] at (0*360/5:0.3) {};
		\node[sn] at (1*360/5:0.3) {};
		\node[sn] at (2*360/5:0.3) {};
		\node[sn] at (3*360/5:0.3) {};
		\node[s4] at (4*360/5:0.3) {};								
	\end{scope}
	
	\begin{scope}[shift={(3*360/5:1.5)}]
		\node[s0] at (0*360/5:0.3) {};
		\node[s1] at (1*360/5:0.3) {};
		\node[sn] at (2*360/5:0.3) {};
		\node[sn] at (3*360/5:0.3) {};
		\node[sn] at (4*360/5:0.3) {};								
	\end{scope}
	
	\begin{scope}[shift={(4*360/5:1.5)}]
		\node[sn] at (0*360/5:0.3) {};
		\node[s1] at (1*360/5:0.3) {};
		\node[s2] at (2*360/5:0.3) {};
		\node[sn] at (3*360/5:0.3) {};
		\node[sn] at (4*360/5:0.3) {};								
	\end{scope}
	
	
	\begin{scope}[shift={(0*360/5:3.0)}]
		\node[sn] at (0*360/5:0.3) {};
		\node[s1] at (1*360/5:0.3) {};
		\node[sn] at (2*360/5:0.3) {};
		\node[sn] at (3*360/5:0.3) {};
		\node[s4] at (4*360/5:0.3) {};								
	\end{scope}
	\begin{scope}[shift={(1*360/5:3.0)}]
		\node[s0] at (0*360/5:0.3) {};
		\node[sn] at (1*360/5:0.3) {};
		\node[s2] at (2*360/5:0.3) {};
		\node[sn] at (3*360/5:0.3) {};
		\node[sn] at (4*360/5:0.3) {};								
	\end{scope}	
	\begin{scope}[shift={(2*360/5:3.0)}]
		\node[sn] at (0*360/5:0.3) {};
		\node[s1] at (1*360/5:0.3) {};
		\node[sn] at (2*360/5:0.3) {};
		\node[s3] at (3*360/5:0.3) {};
		\node[sn] at (4*360/5:0.3) {};								
	\end{scope}	
	\begin{scope}[shift={(3*360/5:3.0)}]
		\node[sn] at (0*360/5:0.3) {};
		\node[sn] at (1*360/5:0.3) {};
		\node[s2] at (2*360/5:0.3) {};
		\node[sn] at (3*360/5:0.3) {};
		\node[s4] at (4*360/5:0.3) {};								
	\end{scope}	
	\begin{scope}[shift={(4*360/5:3.0)}]
		\node[s0] at (0*360/5:0.3) {};
		\node[sn] at (1*360/5:0.3) {};
		\node[sn] at (2*360/5:0.3) {};
		\node[s3] at (3*360/5:0.3) {};
		\node[sn] at (4*360/5:0.3) {};								
	\end{scope}									
\end{tikzpicture}
